Complexity Classification in Infinite-Domain Constraint Satisfaction

A constraint satisfaction problem (CSP) is a computational problem where the input consists of a finite set of variables and a finite set of constraints, and where the task is to decide whether there exists a satisfying assignment of values to the variables. Depending on the type of constraints that we allow in the input, a CSP might be tractable, or computationally hard. In recent years, general criteria have been discovered that imply that a CSP is polynomial-time tractable, or that it is NP-hard. Finite-domain CSPs have become a major common research focus of graph theory, artificial intelligence, and finite model theory. It turned out that the key questions for complexity classification of CSPs are closely linked to central questions in universal algebra. This thesis studies CSPs where the variables can take values from an infinite domain. This generalization enhances dramatically the range of computational problems that can be modeled as a CSP. Many problems from areas that have so far seen no interaction with constraint satisfaction theory can be formulated using infinite domains, e.g. problems from temporal and spatial reasoning, phylogenetic reconstruction, and operations research. It turns out that the universal-algebraic approach can also be applied to study large classes of infinite-domain CSPs, yielding elegant complexity classification results. A new tool in this thesis that becomes relevant particularly for infinite domains is Ramsey theory. We demonstrate the feasibility of our approach with two complete complexity classification results: one on CSPs in temporal reasoning, the other on a generalization of Schaefer's theorem for propositional logic to logic over graphs. We also study the limits of complexity classification, and present classes of computational problems provably do not exhibit a complexity dichotomy into hard and easy problems.

==> design.tex <==
% Things that will be omitted: 
% the classification for (R,+), for its affine variant, 
% the semi-algebraic stuff, and paper with Gustav, mit Feder
% (since not universal-algebraic)
% the phylogenetic classification (because not finished)
% the Junker paper (not yet relevant, needs to be pushed further)




% Design decisions: 

% "False"
% three possibilities: A allow it in fo logic, B consider 0-ary maps for preservation,
% C restrict the preservation theorems
% I list weak and strong points:
% (A) bad:
% problems with defining the canonical database
% apparently, Hodges did it differently (remember issue about QE for non-sentences!)
%
% good:
% the issues in the other solutions are worse.
% could simply restrict the def of canonical database to formulas with at least one 
% variable.
% have similar issue with = in the canonical database! 
% simplifies slightly the QE section
% (B) more work for clones, not nice for the existential positive and the positive 
% preservation theorem: impossible to add some 0-ary preservation there
% (C) not much better is to restrict the preservation theorem to those relations:
% we don't want to distract the reader at that point.

% put gcsp before tcsp: reasons: tcsp is with those "interior automorphisms" the
% more complicated setting, the algorithms are more complicated, it shows
% that things are more complicated if one thinks from the gcsp project
% that everything is very easy

%1 work with finite constraint languages for the CSP, but
% with infinite languages on the mathematical side.

% 2 Focus on results obtained with the universal-algebraic approach

% 3 Focus on omega-categorical structures.
% Therefore, SHOULD mention many qualitative frameworks:
% phylo, branching time, sets, RCC-5, partially ordered time.

% 4 Only relational signatures in the CSP context.
 

% Conventions: 
% use "from xxx" for own publications in theorem heads, and "of xxxx" for publications of others 
% Reihenfolge attribute: Ordered omega-categorical ramsey 
% LATERTD: should settle the issue of "induced substructure" vs  "substructure". Don't need substructures, so probably drop "induced" and define substructures to be induced substructures. 
% Composition: \circ, group actions: \cdot, group multiplication: nothing
% number of variables of an instance: n
% number of constraints of an instance: m
% 3) domain elements: a,b,c,d -- but a might also be an automorphism
% 2) operations: e,f,g,h
% 1) solution maps: s,t -- but these are also tuples
% 24) strings: s  %% could replace by "w" (for word) TD
% 23) variables: x,y,z
% 18) Variable sets: V,W
% 19) Graphs: G,H (shouldn't we make it \mathfrak? may be not - the point is that the signature is simple and 
% the hole thing is simple
% so that it should not have a fancy heavy symbol. It also looks nicer the light way). However, there is additional overlap with $G$
% as a group (which might be curly, though?)
% 22) Digraph: D (shouldn't we make it \mathfrak? may be not) 
% 8) relations: R,S,T,C
% 27) trees, tournaments: T (shouldn't we make it \mathfrak? may be not)
% 28) machines: M
% 29) reductions: R
% 30) special relations: E_3: x=y \neq z OR x \neq y = z
% R^min (temporal relation of special importance)
% Betw, Sep, Cycl, OIT, NAE
% Algebra homomorphisms: \xi (greek analog to h)

% 5) automorphisms: alpha,beta
% CONTRA: 
% a) using a,b,c or g,h instead is more consistent (automorphisms are special polymorphisms) -- look e.g. at the tractability conjecture.
% b) we already use greeks for meta things: formulas, signatures, solutions etc  -- well, but solutions don't really count here, and formulas and 
% signatures come from a different range of symbols
% c) in group theory, having greeks for group elements is highly unusual. 
% AH but here you also shouldn't use greeks, but small romans,
% since we have structures here.
% PRO
% a) it optically makes the terms read nicer. Look e.g. at back-and-forth
% systems 
% b) it puts emphasize on the fact that autos really take a special role
% in practice.
%
% 9) formulas, pp-definitions: \delta, \eta, \gamma. 
% \delta already used for domain formula, so let \gamma 
% be the "generic constraint" (gamma = c = constraint)
% 4) signature: \sigma,\tau
% 31) congruences: big romans would is better.
% 7) formulas: phi,psi   -- I suggest to use it for sentences and
% instances of the CSP. 
% 26) \omega,\kappa: cardinalities
% 6) instances: Phi,Psi  -- SNP sentences
% Theories: S,T,U.
% 10) Generic finite structures: \bA,\bB,\bC,\bD: finite structures
% 11) Generic instance structure: \bA, generic finite structure
% 12) Generic template: \bB (with domain B for "base")
% 13) Generic base structure: \cC 
% whenever we have to choose between \bA,\bB,\bC for
% infinite structures, choose \bB for the thing that you imagine
% as the template of the CSP. 
% E.g., say that $\bB$ is the core of \bA,
% say that \bB has a definition in \bC, etc.

% CHANGE FONTS TO MICHAEL SPECIAL FONT:
% 14) Generic clone: \cC
% 15) Generic function set: \cF
% 16) Generic automorphism group: \cG
% 25) Set of all operations: \mathcal O
% Pro: already have it, stresses non-abstract character of those objects
% Contra: they are typically over a fixed domain (and if not, the action terminology is more appropriate anyhow)
% so the point of introducing a new font to still have the symbol for the domain is pointless. 
% already have the distinction to an abstract group by making the abstract group \bf
% would have to make some domains of abstract groups curly?
% Get confusion between the two ways of making things curly
% Use typical letters anyway, such as C for clones, M for transformation monoids, and G for groups, F for functions, O for operations etc
 
% 17) classes of structures: \mathcal S, \mathcal C, \mathcal A,
% and, relatedly, computational problems \mathcal P, and formal languages \mathcal L.
% 18) sets of forbidden structures: (\mathcal F), \mathcal N
% 19) varieties of algebras (again, these are classes!): \mathcal V
%
% 17) Generic algebra: \bold A, \bold B, \bold C
%
% 20) Special mathematical domains: \mathbb C, \mathbb Q, \mathbb N,
% \mathbb Z, \mathbb R
% 
% Hyphen: inter-definable, bi-interpretable





==> ecsp/feasible-independence.tex <==
\section{Feasible Independence}
Many CSPs with a template $\bB$ having a binary injective polymorphism can be solved in polynomial time
by a certain type of algorithm, which will be formalized in the following. This technique will be used several times
in Chapter~\ref{chap:tcsp} and Chapter~\ref{chap:schaefer}.


\begin{definition}\label{def:feasible-indep}
Let $\bB$ be a relational %an $\omega$-categorical 
structure. We say that $\bB$ has the \emph{feasible independence property}  if $\bB$ has a binary injective polymorphism and there exists a polynomial-time algorithm that returns for a given instance $\bA$ of $\bB$ either 
\begin{enumerate}
%\item \emph{`has injective solution'} when $\bA$ has an injective solution.
\item two elements $a,a'$ of $\bA$ such that $f(a)=f(a')$ for every homomorphism from $\bA$ to $\bB$, or
\item \emph{`injective solution or satisfiable'} when $\bA$ has an injective solution, or no solution.
\end{enumerate}
\end{definition}
Note that Proposition~\ref{prop:injective-sols}, for every input $\bA$ there is indeed a valid output (1) or (2) as in Definition~\ref{def:feasible-indep}. 
It turns out that for structures $\bB$ with the feasible independence property we can reduce $\Csp(\bB)$ to the CSP of the \emph{injectivization} of $\bB$. 
To formally define this concept we need a sequence of definitions.


%\begin{proposition}\label{prop:feasible-indep-alg}
%Suppose $\bB$ has the feasible independence property,
%and let $\bC$ be the injectivization of $\bB$. 
%Then there is a polynomial-time reduction from $\Csp(\bB)$ 
%to $\Csp(\bC)$. 
%\end{proposition}





==> gcsp/old/old.tex <==

Since $\bD$ is definable in the structure $(D;=)$ 
it follows from Theorem~\ref{thm:ecsps} 
that it has a polymorphism which is either a constant or a binary injection.
The former case is impossible as otherwise also $\bB$ has a constant polymorphism by composing the constant of $\bD$ with $e_E$. Let thus $g(x,y)$ be the binary injection 
on $D$ which is a polymorphism of $\bD$. Then $h(x,y):=g(e_E(x),e_E(y))$ is a polymorphism of $\bB$. But $h$ is a binary canonical injection which is $E$-constant, 
and hence $\cC$ contains the operation from case~$(\ref{mt:Nfanatic})$ of our list.
 The argument when $\cC$ contains $e_N$ is identical. 



\begin{definition}\label{defn:bijunctive}
    A relation $R$ on $(\mV;E)$ is called \emph{graph bijunctive}
    if it can be defined in $(\mV;E)$ by a conjunction of disjunctions of disequalities, and of formulas of the form
    \begin{align*}
    x_1 \neq y_1 \; \vee & \; \cdots \; \vee \; x_k \neq y_k \\
    \vee & \; \big (u_1 \neq v_1 \wedge u_2 \neq v_2 \wedge ( X(u_1,v_1) \vee Y(u_2,v_2) ) \big ) \\
    \vee & \; (u_1=v_1 \wedge u_2 = v_2) \; ,
    \end{align*}
    where $X,Y \in \{E,N\}$, variables need not be distinct, and
    $k$ can be $0$.
\end{definition}

\begin{proposition}\label{prop:syntax-graph-bijunctive}
    Let $R$ be a relation with a first-order definition in $(\mV;E)$.
    Then the following are equivalent.
    \begin{enumerate}
        \item $R$ is graph bijunctive;
        \item $R$ is preserved by every straight function of type majority;
        \item $R$ is preserved by a function of type majority and a balanced injection of type $p_1$.
    \end{enumerate}
\end{proposition}

\begin{proof}
    The proof is very similar to the proof
    of Proposition~\ref{prop:syntax-graph-affine}.
    We first show the implication from 1 to 2, that relations that are graph bijunctive
    are preserved by straight functions $f$ of type majority.
    By injectivity of $f$, it suffices to show this for
    the case that the formulas do not contain disequality disjuncts
    (i.e., $k=0$).
    Since the clauses $\phi$ of such a formula
    are such that $\Bool(\phi)$ is bijunctive,
    the claim follows from the fact that bijunctive Boolean relations
    are preserved by the Boolean majority operation
    in very much the same way as in Proposition~\ref{prop:syntax-graph-affine}.

    For the implication from 2 to 3, observe that straight functions of type majority exist since $(\mV;E)$ is universal, and that identifying two variables of such an operation yields a balanced injection of type $p_1$.

    We show the implication from 3 to 1 by induction on the arity
    $n$ of the relation $R$.
    Let $(\mV;E)$ be the balanced binary injection of type $p_1$,
    and let $h$ be the operation of type majority.
    For $n=2$ the statement of the proposition holds because all binary
    relations with a first-order definition over $(\mV;E)$ can be defined as in Definition~\ref{defn:bijunctive}.
    \begin{itemize}
    \item for $\neg E(x,y)$ we can set $k=0$, $X=Y:=N$, $u_1=v_1:=x$,
    $u_2=v_2:=y$; dually, $\neg N(x,y)$ can be defined;
    \item For $x \neq y$, this is trivial;
    \item $E(x,y)$ can be defined as the conjunct of $x\neq y$ and $\neg N(x,y)$; dually, we can define $N(x,y)$;
    \item The relation $x=y$ can be obtained as the conjunction of $\neg E(x,y)$ and $\neg N(x,y)$;
    \item The empty relation is obtained as the conjunction of $E(x,y)$ and $N(x,y)$;
    \item Finally, $V^2$ can be defined by the empty conjunction.
    \end{itemize}

    For $n>2$, we construct the formula $\phi$ that defines the relation $R(x_1,\dots,x_n)$ as follows.
    If there are distinct $i,j \in \{1,\dots,n\}$ such that for all  tuples
    $t$ in $R$ we have $t_i=t_j$, consider the relation
    defined by $\exists x_i. R(x_1,\dots,x_n)$. This relation is also
    preserved by $(\mV;E)$ and $h$, and by
    inductive assumption has a definition $\Psi$ as required.
    Then the formula $\phi := (x_i = x_j) \wedge \psi$ proves the claim.
    So let us assume that for all distinct $i,j$ 
    there is a tuple $t \in R$
    where $t_i \neq t_j$. Note that since $R$ is preserved by the binary injective operation
    $g$, this implies that $R$ also contains an injective tuple.

    Since $R$ is preserved by a function of type majority,
    the relation $\Bool(\inj(R))$ is preserved by the Boolean majority
    operation, and hence has a definition by a 2SAT formula (Theorem~\ref{thm:schaefer}).
    From this definition it is straightforward
    to obtain a definition $\psi(x_1,\dots,x_n)$ of $\inj(R)$ which is the conjunction
    of $\bigwedge_{1\leq i < j \leq n} x_i \neq x_j$ and of
    formulas of the form $E(u,v)$, $N(u,v)$, or
    $$ X(u_1,v_1) \vee Y(u_2,v_2) \; ,$$
    for $u_1,u_2,v_1,v_2 \in \{x_1,\dots,x_n\}$, and $X,Y \in \{E,N\}$.
    We can assume (by removing successively literals from clauses)
    that this formula is \emph{reduced}, i.e., that each of the conjuncts is such that removing any of its literals
    results in an inequivalent formula.

    For all $i,j \in \{1,\dots,n\}$ with $i<j$,
    let $R_{i,j}$ be the relation that holds for the tuple $(x_1,\ldots,x_{i-1},x_{i+1},\ldots,x_n)$ iff $R(x_1,\dots,x_{i-1},x_j,x_{i+1},\dots,x_n)$ holds. Because also $R_{i,j}$ is preserved by $g$ and $h$, but has arity $n-1$, it has a definition
    $\psi_{i,j}$ as in the statement by inductive assumption.
    We call the conjuncts of $\psi_{i,j}$ also the \emph{clauses}
    of $\psi_{i,j}$. 

    Let $\phi$ be the conjunction composed of conjuncts from the following two groups:
    \begin{enumerate}
        \item $\gamma \vee (x_i \neq x_j)$ for all clauses $\gamma$ of $\psi_{i,j}$ and for all $i < j \leq n$;
        \item when $\eta = (X(u_1,v_1) \vee Y(u_2,v_2))$
        is a conjunct of $\psi$, then
        $\phi$ contains the formula $$(\eta \wedge u_1 \neq v_1 \wedge u_2 \neq v_2) \vee (u_1=v_1 \wedge u_2=v_2) \; .$$
    \end{enumerate}
    Obviously, $\phi$ is a formula in the required form.
    We have to verify that $\phi$ defines $R$.

    Let $t$ be an $n$-tuple such that $t \notin R$.
    If $t$ is injective, then since $t \nin \inj(R)$, 
    it violates a clause of the form
    $X(u_1,v_1) \vee Y(u_2,v_2)$ of $\psi$, and hence it violates the corresponding clause in $\phi$.
    If there are $i,j$ such that $t_i=t_j$
    then the tuple 
    $t^i:=(t_1,\dots,t_{i-1},t_{i+1},\dots,t_n) \notin R_{i,j}$.
    Therefore some clause $\gamma$ of
    $\Psi_{i,j}$ is not satisfied by $t^i$, and $\gamma \vee (x_i \neq x_j)$
    is not satisfied by $t$. Thus, in this case $t$ does not satisfy $\phi$ either.

    It remains to be verified that all $t \in R$ satisfy $\phi$.
    Let $\gamma \vee (x_i \neq x_j)$ be a conjunct of $\phi$ created from some clause $\gamma$ of $\psi_{i,j}$.
    If $t_i \neq t_j$, 
    then $t$ satisfies $x_i \neq x_j$. 
    If $t_i = t_j$, 
    then $(t_1,\dots,t_{i-1},t_{i+1},\dots,t_n) \in R_{i,j}$ 
    and thus this tuple satisfies $\psi_{i,j}$. 
    Hence, $t$ satisfies $\gamma$.
    Now, let $\eta$ be a conjunct of $\phi$ from the second group, so it is of the form
    \begin{align*}
    \eta = \; & \big(u_1 \neq v_1 \wedge u_2 \neq v_2 \wedge (X(u_1,v_1) \vee Y(u_2,v_2)) \big )  \\
    & \vee \; (u_1=v_1 \wedge u_2=v_2 ) \; .
    \end{align*}
    We distinguish three cases.
    \begin{enumerate}
        \item The tuple $t$ satisfies both $u_1=v_1$ and $u_2=v_2$.
        In this case we are clearly
        done since $t$ satisfies the second disjunct of $\eta$.
        \item The tuple $t$ satisfies $u_1 \neq v_2$ and $u_2 \neq v_2$. Then the argument is
        exactly the same as the argument in the proof of Proposition~\ref{prop:syntax-graph-affine}.
        \item The remaining case is that $t$ satisfies $u_1=v_1$ and $u_2 \neq v_2$ (or  $u_1 \neq v_1$ and $u_2 = v_2$, but the proof there is symmetric). 
        %We claim that this case cannot occur.
        If $t$ satisfies $Y(u_2,v_2)$, we are done; 
        so let us assume that
        $t$ satisfies $\neg Y(u_2,v_2)$.
        Since we assumed that $\psi$ is reduced, 
        there exists
        a tuple $s \in \inj(R)$ (and hence in $R$) such that $\neg X(u_1,u_1)$ and $Y(u_1,v_1)$; otherwise, we could have replaced the clause $X(u_1,v_1) \vee Y(u_2,v_2)$ by $X(u_1,v_1)$,
        and obtain a contradiction with the assumption that $\psi$ is reduced.  The tuple $r:=g(t,s)$ is injective, and
        satisfies $\neg Y(u_2,u_2)$
        (since $g$ is of type $p_1$)
        and it also satisfies $\neg X(u_1,v_1)$
        (since $g$ is balanced).
        Since $g$ is injective, we have found a tuple $r \in \inj(R)$
        that does not satisfy $X(u_1,v_1) \vee Y(u_1,v_1)$, a contradiction.
    \end{enumerate}
\end{proof}

Combining the following proposition with Proposition~\ref{prop:syntax-graph-bijunctive} finishes the proof of polynomial-time tractability of case~(e) of Proposition~\ref{prop:higherArity}.

\begin{proposition}\label{prop:alg-majority}
    Let $\bB$ be a structure with a first-order definition in $(\mV;E)$ and a finite relational signature, and 
    suppose that $\bB$ is preserved by a straight function of type majority. Then $\Csp(\bB)$ can be solved in polynomial time.
\end{proposition}
\begin{proof}
    The algorithm for $\Csp(\bB)$ is a straightforward adaptation of the procedure given in Figure~\ref{fig:balanced-minority}, with the difference that
    instead of affine Boolean equation systems we have to solve
    2SAT instances in the inner loop.
\end{proof}


% TODO: add proof of Theorem~ref

%\begin{theorem}\label{thm:sigger-terms}
%Let $\bB$ be a structure with a first-order definition in 
%the countably infinite random graph $(V;E)$.
%Then exactly one of the following holds.
%\begin{itemize}
%\item $\bB$ has one out of 17 at most ternary canonical
%polymorphisms (for a detailed description of those see~\cite{BodPin-Schaefer}), and 
%\item There is a $4$-ary polymorphism $f$ of $\bB$
%and automorphisms $\alpha_1$ and $\alpha_2$ of $(V;E)$ such that for all $x,y \in V$ we have
%$$ f(y,y,x,x)= \alpha_1(f(x,x,x,y)) = \alpha_2(f(y,x,y,x)) \; .$$
%In this case, $\Csp(\bB)$ is in P. 
%\item $\bB$ simulates $(\{0,1\}; \OIT)$. In this case, $\bB$ has a finite-signature reduct $\bB$ such that $\Csp(\bB)$ is NP-complete.
%\end{itemize}
%\end{theorem}



%Recall our convention that we say that $\bB$ \emph{simulates} $(\{0,1\};\OIT)$
%if $(1)$ applies (Definition~\ref{def:simulates}).
% I Don't find it a good idea to introduce names in the situation where we still don't 
% know whether constants are necessary or not -- and moreover, it appears that in 
% this theorem we can talk about pp-interpretatations without passing to the mc core!
% In any case, it makes the impression that the above is the def of simulates, which it
% isn't.
%
%Moreover, canonical operations $f$ over $(\mV;E)$ satisfy
%Equation~(\ref{eq:siggers}) in $(2)$ for some automorphisms $\alpha_1,\alpha_2$ of $(\mV;E)$
%if and only if they satisfy the equations of Siggers terms modulo automorphisms
%of $(\mV;E)$ (Proposition~\ref{prop:push-out}).


%\begin{lemma}
 %   Let $f$ be a binary injection of type $p_2$. If $f$ is not balanced, $E$-dominated, $N$-dominated, of type $E/\id$, or of type $N/\id$, then $f$ is not minimal.
%\end{lemma}
%\begin{proof}
%    By duality.
%\end{proof}

%To summarize, we now re-state and prove Theorems~\ref{thm:mainUnary} and ~\ref{thm:main} in the following
%\begin{theorem}[Summary of Theorems~\ref{thm:mainUnary} and~\ref{thm:main}]
%Any minimal function $e$ on the random graph is equivalent to exactly one of the following operations:
%a constant operation; $e_N$; $e_E$; $-$; $\sw$; or
%\begin{itemize}
%\item[(6)] a binary injection of type $p_1$ that is balanced in both arguments;
%\item[(7)]  a binary injection of type $\max$ that is balanced in both arguments;
%\item[(8)]  a binary injection of type $\max$ that is $E$-dominated in both arguments;
%\item[(9)]  a binary injection of type $p_1$ that is $E$-dominated in both arguments;
%\item[(10)]  a binary injection of type $p_1$ that is balanced in the first
%and $E$-dominated in the second argument;
%\end{itemize}
%or to one of the duals of the last four operations (the operation in (6) is self-dual).
%\end{theorem}
%\begin{proof}
%If $e$ is not essential, then it generates, and hence is equivalent to, a constant operation, $e_N$, $e_E$, $-$ or $\sw$; this is the content of Theorem~\ref{thm:mainUnary}, which we already proved in Section~\ref{sect:minimalUnary}. We also have argued that these functions do not generate each other.
%\begin{proof}[Proof of Theorem~\ref{thm:minimalFunctions}]
%By Theorem~\ref{thm:minimalFunctions} it must be canonical and of one of the 9
%types listed there; moreover, Theorem~\ref{thm:minimalFunctions} also shows that
%functions of different types do not generate each other. Observe that in Theorem~\ref{thm:minimalFunctions}, class (1) is (6) here, (2) is (7) here, (3) is the dual of (7) here, (4) is (8) here, (5) is the dual of (8) here, (6) is (9) here, (7) is the dual of (9) here, (8) is (10) here, and (9) is the dual of (10) here.
%\end{proof}



Let $R$, $k$, $r$, $s$, $p_1,\dots,p_r$, $l$ as in the proof of Lemma~\ref{lem:mixtyp:pp}, and we again want to construct a sequence $t^0,t^1,\dots,t^l$ as above. 

For the base case of the induction, $t^0 = h_a(r,s)$ satisfies the requirements since
$h_a$ is injective. For the inductive step, 
suppose that we have already constructed $t^m$,
and that we want to find $t^{m+1}$.
Consider first the case that $N(r_i,r_j)$ for $(i,j)=p_{m+1}$.
Let $\alpha$ be an automorphism that maps $r_i$ to $a$.
 Then $t^{m+1} := h_a(\alpha r,t^m)$ satisfies the requirements.
 If $N(s_i,s_j)$, let $\alpha$ be an automorphism such that 
 $a \notin \{\alpha s_i,\alpha s_j\}$. Then $t^{m+1} := h_a(t^m,\alpha s)$ satisfies the requirements. If none of the two cases applies, then $t^{m+1}=t^m$ satisfies
 the requirements. As explained in Lemma~\ref{lem:mixtyp:pp}, this proves the statement. 


==> tcsp/concl.tex <==
\subsection{Concluding Remarks}
We have completely classified the complexity of the constraint satisfaction problem for temporal constraint languages. By Theorem~\ref{thm:set-trans}, temporal constraint languages are precisely the highly set-transitive structures; hence, we have obtained a complexity  classification for the CSP of those templates
that have in a certain sense that largest possible degree of symmetry.
% with the largest possible degree of symmetry on finite subsets of the template.

See Figure~\ref{fig:summary} for an overview over the nine 
largest tractable temporal constraint languages; the entries also 
mention \emph{typical relations} for the respective
language, i.e., a set of relations that is contained in the language, but not contained in any other of the nine languages -- hence, these
relations show that all the languages are distinct.


\begin{figure}[h]
\begin{center}
\begin{tabular}{|llll|}
\hline
Polymorphism & Typical Relations & Complexity & Reference \\
\hline
min & $\{U,<\}$ & $O(n^2m)$ & Theorem~\ref{thm:min-alg} \\
mi & $\{I \}$ & $O(n^3m)$ & Theorem~\ref{thm:mi-alg} \\
mx & $\{X\}$ & $O(n^4)$ & Theorem~\ref{thm:mx-alg} \\
max = dual min & $\{-U,<\}$ & $O(n^2m)$ & \\
dual mi & $\{-I\}$ &  $O(n^3m)$ & \\
dual mx & $\{-X\}$ & $O(n^4)$ &  \\
ll & $\{(u \neq v) \vee x > y \vee x > z\}$ & $O(nm)$ & Theorem~\ref{thm:ll-alg} \\
dual ll & $\{(u \neq v) \vee x < y \vee x < z\}$ & $O(nm)$  & \\
constant & $\{(x \leq y \leq z) \vee (z \leq y \leq x)\}$ & $O(m)$ & \\
\hline
\end{tabular}
\caption{Summary of the various tractable languages. For the last three operations, the typical relations are given by their first-order definition; in all other cases, see Section~\ref{sect:shuffle}.}
\label{fig:summary}
\end{center}
\end{figure}


Finally, we would like to remark that it follows from the descriptions of the constraint languages via the polymorphisms given in the paper
that the so-called \emph{meta-problem} for
tractability is decidable; this is formally stated in the following
corollary.

%TODO: rework this in the light of the general decidability results
\begin{corollary}
Let $\bB = (\mathbb Q; R_1,\dots,R_n)$ be a finite temporal constraint language
and let $\phi_1,\dots,\phi_n$ be quantifier-free first-order formulas
 that define $R_1,\dots,R_n$ over $(\mathbb Q;<)$, respectively.
There is an algorithm that, given $\phi_1,\dots,\phi_n$, decides
whether $\Csp(\bB)$ is tractable or NP-complte.
\end{corollary}
\begin{proof}
Theorem~\ref{thm:main} shows that it suffices to test for each of the nine (at most binary) polymorphisms whether all relations $R_1,\dots,R_n$ are preserved by this polymorphism.
Suppose that $R_i$ is $k$-ary.
Clearly, whether or not a $k$-tuple $t \in \mathbb Q^k$ is in $R_i$
only depends on the weak linear order $\preceq$ of the entries of $t$.
Now observe that for $f \in \{\min, \mi, \mx, \max, \dmi, \dmx\}$ 
the weak linear order of the $k$-tuple $f(t_1,t_2)$ 
is determined by the weak linear order of the $2k$-tuple $(t_1,t_2)$. 
Hence, to test whether $R_i$ is preserved by $f$ it
suffices to verify for a finite number of
weak linear orders whether they satisfy $\phi_i$.
A procedure that decides whether $R_i$ is preserved by
\lele\  or \dll\  has been described in~\cite{ll}.
Testing whether $R_i$ is preserved by a constant polymorphism
is trivial, we only have to verify whether the $k$-tuple $(0,\dots,0)$
satisfies $\phi_i$.
\end{proof}


==> tcsp/general.tex <==
\section{The complete classification}
\label{sec:lcsp-classif}
Temporal constraint languages where not all first-order definable relations are primitive positive definable can be divided into four (non-disjoint) groups: those preserved by a constant operation, 
by \pp, by \dpp, or by an operation called \lex, which will be introduced
in the next subsection\footnote{In the terminology of~\cite{maximal}, the operations \pp, \dpp, and \lex\ define \emph{maximal}
constraint languages.}. 
%These groups are orthogonal to Cameron's
%classification: there are first-order interdefinable temporal constraint
%languages $\Gamma$ and $\Gamma'$ such that 
%$\Gamma$ is preserved by
%one of the above operations and $\Gamma'$ is not. On the other hand,
%two structures that are not first-order interdefinable might both be
%preserved by \lex\ and not by \pp\ and \dpp. 
None of the three polymorphisms \pp, \dpp, and \lex\ alone guarantees tractablility of CSP$(\Gamma)$. An illustration of the classification result for the languages that preserve $<$ can be found in Figure~\ref{fig:tcsp-simple}.

\input tcsp/ll.tex
\input tcsp/gen-ll.tex
\input tcsp/classification.tex

==> tcsp/injective.tex <==
\section{The Injective Case}
This section treats a subclass of temporal CSPs
that has been called \emph{ordering constraints} 
in the literature on random CSPs, and in the literature on approximation ratios
for MaxCSPs. % TODO: make sure that MaxCSPs are defined. 
The corresponding temporal constraint languages only contain \emph{injective}
temporal relations; recall from Definition~\ref{def:injective} that a relation $R$ is injective
if every tuple in $R$ only contains tuples with pairwise distinct entries. 
For injective languages, the classification result is substantially simpler to show;
at the same time, the results of this section will be useful to obtain the full classification.
We will prove the following.

\begin{theorem}
Let $\bB$ be an injective temporal constraint language that contains $<$. 
Then either $\Betw$ has a primitive positive definition in $\bB$, and $\Csp(\bB)$ is NP-hard, or all relations in $\bB$ can be defined by conjunctions of
clauses of the form $z_0 > z_1 \vee \dots \vee z_0>z_l$ and of the form $x \neq y$. 
\end{theorem}

We again use the concept of \emph{behavior} of operations over a relational structure;
note that a $k$-ary operation
$f$ behaves like a $k$-ary operation $g$ on $S = S_1 \times \cdots \times S_k$
if for all $t,t' \in S$ we have $f(t) \leq f(t')$ iff $g(t) \leq g(t')$. That is, the weak linear order induced by $f$ on the tuples from $G$ (in the sense of Observation~\ref{obs:f-gen-g-order}) is the same as the weak linear order induced on these tuples by $g$.
A $k$-ary operation $f: \mathbb Q^k \rightarrow \mathbb Q$
is \emph{dominated} by the $i$-th argument when for all $a, b \in \mQ^k$
it holds that
$f(a_1,\dots,a_k) \leq f(b_1,\dots,b_k)$ if and only if $a_i \leq b_i$.
Let $\mQ^+$ denote the set of all positive rational numbers, and let $\mQ^-_0$ denote $\mQ \setminus \mQ^+$.

\begin{definition}\label{def:merge}
Let $f,g$ be from $\mQ^2 \rightarrow \mathbb Q$. 
Then $[f|g]$ denotes an arbitrary operation  from $\mathbb Q^2 \rightarrow \mathbb Q$ with the following
properties. For all $x,x',y,y' \in \mathbb Q$,
\begin{itemize} 
\item if $x \leq 0$ and $x' > 0$ then $[f|g](x,y) < [f|g](x',y')$;
\item $[f|g]$ behaves like $f$ on $\mathbb Q^-_0 \times \mathbb Q$;
\item 
$[f|g]$ behaves like $g$ on $\mathbb Q^+ \times \mathbb Q$;
\end{itemize}
\end{definition}

We first present a syntactic result for injective temporal relations that are preserved
by an operation $[f|g]$ where $f$ is dominated by the first argument and $g$ is dominated by the second argument. 

\begin{proposition}\label{prop:syntax}
Let $f,g$ be binary polymorphisms of $(\mQ;\leq)$ such that $g$ is dominated by the second argument. 
Let $R$ be an injective temporal relation that is preserved by $[f|g]$.
Then $R$ has a definition by a conjunction of
clauses of the form $z_0 > z_1 \vee \dots \vee z_0>z_l$ and of the form $x \neq y$. 
\end{proposition}

We present the proof of Proposition~\ref{prop:syntax} as a consequence of 
Lemma~\ref{lem:inj} below, which is more flexible for later use since it applies
to arbitrary temporal relations, not just to injective ones.  
Note that every temporal relation $R$
can be defined by a quantifier-free formula in conjunctive normal
form where all literals are of the form $x > y$ or $x=y$;
to see this, take any quantifier-free formula in conjunctive
normal form that defines $R$ over $({\mathbb Q};<)$ and 
\begin{itemize}
\item replace $\neg (x < y)$ by the two literals $(x > y) \vee (x=y)$;
\item replace $x \neq y$ by the two literals $(x > y) \vee (y > x)$;
\item replace $x < y$ by $y > x$.
\end{itemize}
We call formulas in quantifier-free conjunctive normal form where all literals are of the form $x>y$ or $x=y$ \emph{standard formulas}.
A clause is \emph{bad} if it is not of the form $z_0 > z_1 \vee \dots \vee z_0> z_l$.

\begin{lemma}\label{lem:inj}
Let $R$ be a temporal relation. 
If $R$ is preserved by the operation $[f|g]$ from Proposition~\ref{prop:syntax},
then there is a standard formula without bad clauses such that
an injective tuple is in $R$ if and only if it satisfies $\phi$. 
\end{lemma}

\begin{proof}
Suppose that $R$ is $n$-ary. Let $\phi$ be a standard formula 
such that an injective tuple is in $R$ if and only if it satisfies $\phi$;
choose $\phi$ in such a way that 
it has a minimal number of bad clauses. 
We can assume without loss of generality that $\phi$ does not contain
literals of the form $x=y$; otherwise, we can simply remove those literals
and work with the resulting formula instead. 
Suppose for contradiction that $\phi$ contains a bad clause $C$.
Then $C$ must contain two literals 
$l_1 := u > v$ and $l_2 := r > s$ where $u$ and $r$ are distinct variables. 
Let $V$ be the set of variables of $\phi$.
We claim that $\phi$ has an injective satisfying assignment 
$i_1: V \rightarrow \mQ$ 
such that $l_1$ is the only literal satisfied by $i_1$ in $C$. 
Otherwise, the formula obtained
from $\phi$ by removing $l_1$ from $C$ still has the property
that every injective tuple is in $R$ if and only if it satisfies $\phi$.
Moreover, the number of bad clauses in the new formula is also minimal,
which is impossible by the choice of $\phi$.
Similarly one can see that $\phi$ has an injective satisfying assignment 
$i_2: V \rightarrow \mQ$ such that $l_2$ is the only literal satisfied by $i_2$ in $C$.

Suppose for contradiction that 
$i_1$ can be chosen such that $i_1(r)$ is smaller than $i_1(s)$, $i_1(u)$, and $i_1(v)$. 
Let $\alpha \in \AQ$ be such that $\alpha i(r)=0$. Consider
the mapping $i_0: V \rightarrow \mQ$ defined by $i_0(x) = [f|g](\alpha i_1(x),i_2(x))$. 
If a literal in some clause of $\phi$ is not satisfied in both tuples $t_1$ and $t_2$,
then it is also not satisfied in $t$, because $[f|g]$ and $\alpha$ preserve $\leq$. 
Therefore $l_1$ and $l_2$ are the only literals of $C$ satisfied by $i_0$
Since $i_0(r)$ is strictly smaller than $i_0(s)$, 
the literal $l_2$ cannot be satisfied by $i_0$. Since $i_2(v) > i_2(u)$ and $g$ is dominated by the second argument, it also holds
that $i_0(v)>i_0(u)$, and hence $l_1$ is not satisfied in $i_0$ either.
So $i_0$ does not satisfy $\phi$, 
in contradiction to the assumption that $R$ is preserved by $[f|g]$.

An analogous argument shows that $i_2$ cannot be chosen such 
that $i_2(u)$ is smaller than $i_2(v)$, $i_2(r)$, and $i_2(s)$. 
We claim that all injective satisfying assignments $j: V \rightarrow \mQ$ 
of $\phi$ also satisfy $(u > v) \vee (u > s)$.
Otherwise, $j(u) < j(v)$ and $j(u) < j(s)$,
therefore $j(u) > j(r)$ to satisfy the property from the beginning of the paragraph. 
Hence, $j(r)<j(v)$ and $j(r) < j(s)$.
But then $j(r)$ is smaller than $i_2(v)$, $i_2(r)$, and $i_2(s)$,
in contradiction to what we have shown before.
Analogously we can show that any injective satisfying assignment of
$\phi$ also satisfies $(r > v) \vee (r > s)$.


Let $\phi'$ be the formula obtained from $\phi$ by removing $C$ and adding
the two clauses $(u > v) \vee (u > s)$ and $(r > v) \vee (r > s)$. We show that an injective tuple satisfies $\phi'$ 
if and only if it satisfies $\phi$. By what we have seen above, 
it suffices to show that $\phi'$ implies $\phi$.
Let $j$ be any satisfying assignment of $\phi'$. Clearly,
all the clauses of $\phi$ except for $C$ are satisfied by $j$, because
they are also present in $\phi'$. 
We can reformulate the two additional clauses in $\phi'$ to 
$$ (u > v \wedge r > v) \vee (u > v \wedge r > s)
\vee (u  > s \wedge r > v) \vee (u > s \wedge r > s) \; .$$ 
If the first, the second, or the fourth disjunct is satisfied by $j$, then 
$j(u) > j(v) \; \vee \; j(r) > j(s)$, and therefore $C$ holds in $j$.
If the third disjunct is satisfied by $j$ and the literal $l_1$ does not
hold (i.e., $j(u)<j(v)$), we have the chain of inequalities $j(s)<j(u)<j(v)<j(r)$ and hence $l_2$ is satisfied.  
The formula $\phi'$ has fewer bad clauses than $\phi$, contradicting the choice of $\phi$.
\end{proof}

Proposition~\ref{prop:syntax} follows, since we can apply Lemma~\ref{lem:inj},
to $R$ to obtain a formula $\phi$ without bad clauses; the formula $\phi \wedge \bigwedge_{x,y \in V} x \neq y$ then defines $R$ and is of the desired form.
The goal in the following is to prove that if $\Betw$ does not have a primitive positive
definition in $\bB$, then $\bB$ has a polymorphism of the form $[f|g]$ as described in 
Proposition~\ref{prop:syntax}. 

\begin{lemma}\label{lem:lcsp-viol-btw-inj-tuples}
Let $f$ be a binary operation violating \btw\ and preserving $<$. Then
there are $t_1,t_2\in\btw$ such that $f(t_1,t_2)$
has three distinct entries and $f(t_1,t_2)\not\in\btw$.
\end{lemma}
\begin{proof}
Since $f$ violates \btw, there are two triples $t_1,t_2\in\btw$ such
that $t:=f(t_1,t_2)\not\in\btw$.  Because $f$ preserves $<$, we 
can assume without loss of generality that
$t_1[1]<t_1[2]<t_1[3]$ and $t_2[1]>t_2[2]>
t_2[3]$. If $t$ has three distinct entries (in this case, 
we also say that $t$ is injective), we are done. Otherwise
we distinguish two cases:
\begin{enumerate}
\item $t[1]=t[2]=t[3]$: In that case, take a triple $s_1$
such that $s_1[1]<t_1[1]$, $s_1[2]=t_1[2]$, and
$s_1[3]=t_1[3]$. We also choose a triple $s_2$ such that
$t_2[2]<s_2[1]<t_2[1]$, $s_2[2]=t_2[2]$, and
$s_2[3]=t_2[3]$. It is straightforward to check that $s_1[1]<
s_1[2]<s_1[3]$ and $s_2[1]>s_2[2]>s_2[3]$ and thus
both triples belong to \btw. Now, consider $s:=f(s_1,s_2)$.
We have that $s[2]=t[2]$,
$s[3]=t[3]$, and $s[1]<t[1]=s[2]=s[3]$ because $f$ preserves $<$.
Therefore $s\not\in\btw$.  Take $s_1$ instead of $t_1$,
$s_2$ instead of $t_2$ and proceed with case 2.
\item If exactly two entries in $t$ have the same value, let $i,j$ be
their indices and let $k$ be the index of the entry with the unique value.  We
assume that $t[k]>t[i]$ (the other case is symmetric). It is
straightforward to verify that there is an entry in $t$ such that making
the value of this entry smaller would make $t$ injective and it would still
not be in \btw. We can assume without loss of generality that $i$ is an index
of such an entry. We choose $s_1$ so that $s_1[i]<t_1[i]$,
$s_1[j]=t_1[j]$, $s_1[k]= t_1[k]$, and
$s_1[1]<s_1[2]<s_1[3]$. We choose $s_2$ such that
$s_2[i]<t_2[i]$, $s_2[j]=t_2[j]$,
$s_2[k]=t_2[k]$, and $s_2[1]>s_2[2]>s_2[3]$.  Note that $s_1,s_2\in\btw$. The tuple
$s:=f(s_1,s_2)$ satisfies $s[i]<t[i]$,
$s[j]=t[j]$, and $s[k]=t[k]$. By the choice of $i$ we
conclude that $s$ is injective, $s\not\in\btw$ and we are done.
\end{enumerate}
\end{proof}

We use Ramsey theory via Theorem~\ref{thm:higher-ary-canonical-violation}
 to prove the following.

\begin{lemma}\label{lem:lcsp-lex-or-pp}
Let $f$ be a binary operation that preserves $<$ and violates \btw. 
Then $f$ generates an operation $[g_1|g_2]$ for polymorphisms $g_1,g_2$ of $(\mQ;\leq)$ such that $g_2$ is dominated by the second argument.
\end{lemma}


==> tcsp/old.tex <==


\ignore{
Let $R = \{0,1\}^3 \setminus \{(0,0,0)\}$ and $N = \{(0,1),(1,0)\}$.
Then the relation $\NAE(x,y,z)$ has in $(\{0,1\};R,N)$ the primitive positive definition
$$\exists x',y',z' \, \big(N(x,x') \wedge N(y,y') \wedge N(z,z') \wedge R(x,y,z) \wedge R(x',y',z') \big) \; .$$
Hence, by Proposition~\ref{prop:hard-boolean-csps} and Theorem~\ref{thm:simulates-tame}, 
it suffices to prove that $(\{0,1\};R,N)$ has a primitive positive interpretation in 
$({\mathbb Q}; \Cycl)$. 

The idea of the interpretation is inspired by the NP-hardness proof of~\cite{GalilMegiddo} for the `Cyclic ordering problem' (see~\cite{GareyJohnson}).
The dimension of our interpretation $I$ is three, and the domain formula $\delta_I(x_1,x_2,x_3)$ is $x_1 \neq x_2 \wedge x_2 \neq x_3 \wedge x_3 \neq x_1$,
which clearly has a primitive positive definition in $({\mathbb Q}; \Cycl)$.
The coordinate map $h$ sends $(x_1,x_2,x_3)$ to $0$ if
$\Cycl(x_1,x_2,x_3)$, and to $1$ otherwise. Note that
$h(x_1,x_2,x_3)=1$ if and only $\Cycl(x_1,x_3,x_2)$.

Let $\phi(x_1,x_2,x_3,y_1,y_2,y_3)$ be the formula
\begin{align*}
& \Cycl(x_1,y_1,x_2) \wedge \Cycl(y_1,x_2,y_2) \wedge \Cycl(x_2,y_2,x_3) \\
& \Cycl(y_2,x_3,y_3) \wedge \Cycl(x_3,y_3,x_1) \wedge \Cycl(y_3,x_1,y_1)  \; .
\end{align*}
When $(a_1,\dots,a_6)$ satisfies $\phi$, we can imagine $a_1,\dots,a_6$ as points that appear clockwise in this order on the unit circle.
In particular, we then have that $\Cycl(a_1,a_3,a_5)$ holds if and only if $\Cycl(a_2,a_4,a_6)$ holds. 
The formula $=_I(x_1,x_2,x_3,y_1,y_2,y_3)$ is
\begin{align*}
\exists u^1_1,\dots,u^4_3 \, & \big ( \phi(x_1,x_2,x_3,u^1_1,u^1_2,u^1_3) \\
\wedge \; & \bigwedge_{i=1}^3 \phi(u^i_1,u^i_2,u^i_3,u^{i+1}_1,u^{i+1}_2,u^{i+1}_3) \\ 
\wedge \; & \phi(u^4_1,u^4_2,u^4_3,y_1,y_2,y_3) \big )
\end{align*}
which is equivalent to $\delta(x_1,x_2,x_3) \wedge \delta(y_1,y_2,y_3) \wedge (\Cycl(x_1,x_2,x_3) \Leftrightarrow \Cycl(y_1,y_2,y_3))$.
To see this, suppose that $(a_1,a_2,a_3,b_1,b_2,b_3) \in {\mathbb Q}^6$ satisfies $=_I$, and suppose that $(a_1,a_2,a_3) \in \Cycl$. Then the conjunct $\phi(x_1,x_2,x_3,u^1_1,u^1_2,u^1_3)$ of $=_I$ implies that $\Cycl(u^1_1,u^1_2,u^1_3)$. 
The conjunct $\phi(u^i_1,u^i_2,u^i_3,u^{i+1}_1,u^{i+1}_2,u^{i+1}_3)$ implies
that $\Cycl(u^{i+1}_1$,
$u^{i+1}_2,u^{i+1}_3)$, for all $i \leq 3$, and so by the last conjunct 
we finally conclude that $\Cycl(b_1,b_2,b_3)$. The same reasoning shows that
$=_I(a_1,a_2,a_3,b_1,b_2,b_3) \wedge \Cycl(b_1,b_2,b_3)$ implies $\Cycl(a_1,a_2,a_3)$. 

Conversely, if
we have $\Cycl(a_1,a_2,a_3)$ and $\Cycl(b_1,b_2,b_3)$ then
we can select points
for $u_1^1,\dots,u_3^4$ that show that 
$=_I(a_1,a_2,a_3,b_1,b_2,b_3)$ is satisfiable, as follows.
We only consider orders on $a_1,a_2,a_3,b_1,b_2,b_3$ that start with $a_1$; this is without loss of generality, since $\Cycl$ is preserved by $\cyc$.

\begin{figure}
\begin{center}
\begin{tabular}{l|l}
\hline
Cyclic order on $(\bar a, \bar b)$ & How to set $u^1_1,\dots,u^4_3$ \\
\hline \hline 
$a_1 < a_2 < a_3 < b_1 < b_2 < b_3$ & $a_1 < u^1_1 < a_2 < u^2_1 < u^1_2 < a_3 < u^3_1 < u^4_1 < b_1 $ \\ 
&  $< u^2_2 < u^3_2 < u^4_2 < b_2 < u^1_3 < \dots < u^4_3 < b_3$ \\ % 1
\hline
$a_1 < a_2 < b_1 < a_3 < b_2 < b_3$ & $a_1 < u^1_1 < a_2 < u^2_1 < u^3_1 < u^4_1 < b_1 < u^1_2 < a_3$ \\ 
& $< u^2_2 < u^3_2 < u^4_2 < b_2 < u^1_3 < \dots < u^4_3 < b_3$ \\ % 2
\hline
$a_1 < a_2 < b_1 < b_2 < a_3 < b_3$ & $a_1 < u^1_1 < a_2 < u^2_1 < u^3_1 < u^4_1 < b_1 < u^1_2 < u^2_2$ \\ 
& $< u^3_2 < u^4_2 < b_2 < a_3 < u^1_3 < \dots < u^4_3 < b_3$ \\ % 3
\hline
$a_1 < a_2 < b_1 < b_2 < b_3 < a_3$ & $a_1 < u^4_1 < u^3_2 < u^2_3 < u^1_1 < a_2 < b_1 < u_2^4 < b_2$ \\
& $< u_3^4 < u^4_3 < u^2_1 < u^1_2 < b_3 < a_3 < u_1^3 < u^2_2 < u^1_3$ \\ % 4
\hline
$a_1 < b_1 < a_2 < a_3 < b_2 < b_3$ & $a_1 < u^1_1 < \dots < u^4_1 < b_1 < a_2 < u^1_2 < a_3 <$ \\
& $u^2_2 < u^3_2 < u^4_2 < b_2 < u^1_3 < \dots < u^4_3 < b_3$\\ % 5
\hline
$a_1 < b_1 < a_2 < b_2 < a_3 < b_3$ & $a_1 < u^1_1 < \dots < u^4_1 < b_1 < a_2 < u^1_2 < \dots < u^4_2 <$ \\ 
& $b_2 < a_3 < u^1_3 < \dots < u^4_3 < b_3$ \\ % 6
\hline
$a_1 < b_1 < a_2 < b_2 < b_3 < a_3$ & $a_1 < u^4_1 < b_1 < u^3_2 < u^2_3 < u^1_1 < a_2 < u^4_2 < b_2 <$ \\
& $u^3_3 < u^4_3 < b_3 < u^2_1 < u^1_2 < a_3 < u^3_1 < u^2_2 < u^1_3$ \\ % 7
\hline
$a_1 < b_1 < b_2 < a_2 < a_3 < b_3$ & $a_1 < u^4_1 < b_1 < u^3_2 < u^4_2 < b_2 < u^2_3 < u^1_1 < a_2 <$\\ 
& $u^2_1 <  u^1_2 <  a_3 < u^3_3 < u^4_3 < b_3$ \\ % 8
\hline
$a_1 < b_1 < b_2 < a_2 < b_3 < a_3$ & $a_1 < u^4_1 < b_1 < u^3_2 < u^4_2 < b_2 < u^2_3 < u^1_1 < a_2 < $ \\
& $u^3_3 <  u^4_3 < b_3 < u^2_1 < u^1_2 < a_3 < u^3_1 < u^2_2 < u^1_3 $ \\ % 9
\hline
$a_1 < b_1 < b_2 < b_3 < a_2 < a_3$ & $a_1 < u^3_1 < u^4_1 < b_1 < u^2_2 < u^3_2 < u^4_2 < b_2 < b_3 < $ \\
& $u^1_3 < \dots < u^4_3 < a_2 < u^1_1 < a_3 < u^2_1 < u^1_2$ % 10
\end{tabular}
\end{center}
\caption{Assignments for the correctness of the primitive positive definition of $\phi_=$.}
\label{fig:cyc-gadget}
\end{figure}

The formula $\neg_I(x_1,x_2,x_3,y_1,y_2,y_3)$
is $=_I(x_1,x_2,x_3,z_1,z_3,z_2)$.

The formula
$R_I(x_1,x_2,x_3,y_1,y_2,y_3,z_1,z_2,z_3)$ is
\begin{align*}
\exists a,b,c,d,e,f,g,h,i,j,k,l,m,n \, & \big (\Cycl(a,c,j) \wedge \Cycl(b,j,k) \wedge \Cycl(c,k,l) \\
\wedge \; & \Cycl(d,f,j) \wedge \Cycl(e,j,l) \wedge \Cycl(f,l,m) \\
\wedge \; & \Cycl(g,i,k) \wedge \Cycl(h,k,m) \wedge \Cycl(i,m,n) \\\wedge  \; & \Cycl(n,m,l)
\wedge =_I(x_1,x_2,x_3,a,b,c) \\
\wedge  \; & =_I(y_1,y_2,y_3,d,e,f) \wedge =_I(z_1,z_2,z_3,g,h,i)  \big ) \, .
\end{align*}
The proof that for all tuples $\bar a_1, \bar a_2, \bar a_3 \in
{\mathbb Q}^3$
\begin{align*}
(h(\overline a_1), h(\overline a_3),  h(\overline a_3)) \in R \;
& \Leftrightarrow \;
({\mathbb Q}; \Cycl) \models R_I(\overline a_1, \overline a_2, \overline a_3)
\end{align*}
follows the correctness proof of the reduction presented
in~\cite{GalilMegiddo}.

First, suppose that 
$\bar a_1, \bar a_2, \bar a_3 \in {\mathbb Q}^3$ are such that
$(h(\bar a_1), h(\bar a_2), h(\bar a_3)) \nin R$. 
Hence, $h(\bar a_i)=0$ and $\Cycl(\bar a_i[1],\bar a_i[2],\bar a_i[3])$ for all $i \leq 3$. 
Suppose for contradiction 
that there were values for the variables $a,b,c,d,e,f,g,h,i,j,k,l,m,n$ in 
$R_I$ such that all the conjuncts of $R_I$ are true. 
Then the conjuncts of $R_I$ involving the formula $=_I$ imply that
$\Cycl(a,b,c)$, $\Cycl(d,e,f)$, and $\Cycl(g,h,i)$. 
Then 
\begin{align*} 
&\Cycl(a,b,c) \xrightarrow{\Cycl(a,c,j)} \Cycl(b,c,j) \xrightarrow{\Cycl(b,j,k)} \Cycl(c,j,k) \xrightarrow{\Cycl(c,k,l)} \Cycl(j,k,l) \\
& \Cycl(d,e,f) \xrightarrow{\Cycl(d,f,j)} \Cycl(e,f,j) \xrightarrow{\Cycl(e,j,l)} \Cycl(f,j,l) \xrightarrow{\Cycl(f,l,m)} \Cycl(j,l,m) \\
& \Cycl(g,h,i) \xrightarrow{\Cycl(g,i,k)} \Cycl(h,i,k) \xrightarrow{\Cycl(h,k,m)} \Cycl(i,k,m) \xrightarrow{\Cycl(i,m,n)} \Cycl(k,m,n) \\
& \Cycl(j,k,l) \xrightarrow{\Cycl(j,l,m)} \Cycl(k,l,m) \xrightarrow{\Cycl(k,m,n)} \Cycl(l,m,n) \, .
\end{align*}
But $\Cycl(l,m,n)$ is in contradiction to the conjunct $\Cycl(n,m,l)$.

\begin{figure}
\begin{center}
\begin{tabular}{|l|l|l|}
\hline
$(h(\bar a_1),h(\bar a_2),h(\bar a_3))$ & $\Cycl$ contains & Order on variables \\
%$a,b,c,d,e,f,g,h,i,j,l,m,n$ \\
\hline \hline
%$h(\bar a_1)=1$, $h(\bar a_2)=0$, $h(\bar a_3)=0$ & $\Cycl(a,c,b)$, $\Cycl(d,e,f)$, $\Cycl(g,h,i)$ 
$(1,0,0)$ & $(a,c,b),(d,e,f),(g,h,i)$ & $\overrightarrow{ackmbdefjlnghi}$ \\
%$h(\bar a_1)=0$, $h(\bar a_2)=1$, $h(\bar a_3)=0$ & $\Cycl(a,b,c)$, $\Cycl(d,f,e)$, $\Cycl(g,h,i)$ 
$(0,1,0)$ & $(a,b,c),(d,e,f),(g,i,h)$ 
& $\overrightarrow{abcjkdmflneghi}$ \\
%$h(\bar a_1)=0$, $h(\bar a_2)=0$, $h(\bar a_3)=1$ & $\Cycl(a,b,c)$, $\Cycl(d,e,f)$, $\Cycl(g,i,h)$ 
$(0,0,1)$ & $(a,b,c),(d,e,f),(g,i,h)$ & $\overrightarrow{abcdefjklngimh}$ \\
%$h(\bar a_1)=1$, $h(\bar a_2)=1$, $h(\bar a_3)=0$ & $\Cycl(a,c,b)$, $\Cycl(d,f,e)$, $\Cycl(g,h,i)$ 
$(1,1,0)$ & $(a,c,b),(d,f,e),(g,h,i)$ & $\overrightarrow{ackmbdfejlnghi}$ \\
%$h(\bar a_1)=1$, $h(\bar a_2)=0$, $h(\bar a_3)=1$ & $\Cycl(a,c,b)$, $\Cycl(d,e,f)$, $\Cycl(g,i,h)$ 
$(1,0,1)$ & $(a,c,b),(d,e,f),(g,i,h)$ 
& $\overrightarrow{ackmbdefjlngih}$ \\
%$h(\bar a_1)=0$, $h(\bar a_2)=1$, $h(\bar a_3)=1$ & $\Cycl(a,b,c)$, $\Cycl(d,f,e)$, $\Cycl(g,i,h)$ 
$(0,1,1)$ & $(a,b,c),(d,f,e),(g,i,h)$ & $\overrightarrow{abcjkdmflnegih}$ \\
%$h(\bar a_1)=1$, $h(\bar a_2)=1$, $h(\bar a_3)=1$ & $\Cycl(a,c,b)$, $\Cycl(d,e,f)$, $\Cycl(g,i,h)$ 
$(1,1,1)$ & $(a,c,b),(d,e,f),(g,i,h)$ & $\overrightarrow{acbjkdmflnegih}$ \\
\hline
\end{tabular}
\end{center}
\caption{Assignments for the correctness of the interpretation of $(\{0,1\};\OIT)$ in
$({\mathbb Q}; \Cycl)$. We use the terminology from Section~\ref{ssect:tcsp-aut}.}
\label{fig:correctness-cyc}
\end{figure}

Conversely, suppose that
$\bar a_1, \bar a_2, \bar a_3 \in {\mathbb Q}^3$ are such that
$(h(\bar a_1), h(\bar a_2), h(\bar a_3)) \in R$. Hence, there must be an $i \leq 3$ such that 
$h(\bar a_i) = 1$, and thus $\Cycl(\bar a_i[1],\bar a_i[2],\bar a_i[3])$. We have to
find values for the variables $a,b,c,d,e,f,g,h,i,j,k,l,m,n$ of $R_I$ so that all conjuncts
of $R_I$ are satisfied when evaluated at $\bar a_1, \bar a_2, \bar a_3$. For this, it suffices to specify a linear order on those variables that satisfies all the conjuncts in
$R_I$ so that $\Cycl(\bar a_1[1],\bar a_1[2],\bar a_1[3])$ if and only if $\Cycl(a,b,c)$,
$\Cycl(\bar a_2[1],\bar a_2[2],\bar a_2[3])$ if and only if $\Cycl(d,e,f)$, and
$\Cycl(\bar a_3[1],\bar a_3[2],\bar a_3[3])$ if and only if $\Cycl(g,h,i)$.
Those linear orders can be found in the table of Figure~\ref{fig:correctness-cyc}. 
\end{proof}
}





such that $f(x,y,z) = f(x',y',z')$ if at least one of the following holds. 
\begin{enumerate}
\item $x=x'$, and $y,y' > x$, and $z,z' > x$; 
% x-Platte
\item $y=y'$, and $x,x' > y$, and $z,z' > y$;
% y-Platte
\item $z=z'$, and $x,x' > z$, and $y,y' > z$; 
% z-Platte
\item $y=y'=z=z'$ and $x,x'>z$;
% x-Balken
\item $x=x'=z=z'$ and $y,y'>x$;
% y-Balken
\item $x=x'=y=y'$ and $z,z'>x$; 
% z-Balken
\item $x=x'=y=z'=z=z'$. 
% Diagonale
\end{enumerate}
For a fixed $u$, 

Moreover, $f(x,y,z)<f(x',y',z')$ holds if
at least one of the following holds.
% Eigentlich egal wie, hauptsache
% Balken kommen unter Platten?
% Waehlen also die Ordnung:
% Diagonale < x-Balken < y-Balken < z-Balken
% < x-Platte < Z-Platte < Y-Platte < x-Platte
\begin{itemize}
\item $x=y=z$ and $x < x'$ and $y \leq y'$ and $z \leq z'$; 
% Zwischen Diagonale und naechstem 
% x-Balken
\item $y = z = z' = x'$ and $x > x'$ and $y > y'$; 
% Zwischen x-Balken und entsprechendem
% y-Balken
\item $x = z = x' = y'$ and $y > y'$ and
$z > z'$;
% Zwischen y-Balken und entsprechendem
% z-Balken
\item $x = y = z'$ and $z > z'$ and $x < x'$ and $y < y'$; 
%Zwischen z-Balken und z-Platte
\item $z = y'$ and $x > z$ and $y > z$ and $x' > y'$ and $z' > y'$;
% Zwischen z-Platte und y-Platte
\item $y = x'$ and $x > y$ and $z > y$ and $y' > x'$ 
and $z' > x'$; 
% Zwischen y-Platte und x-Platte. 
\item $x < x'$, $y > x$, $z > x$, $x' \leq y'$, and $x' \leq z'$. 
% Zwischen x-Platte und Diagonale
\end{itemize}
%and $\alpha,\beta \in \Aut%({\mathbb Q};<)$ with the following %properties: 
%$f$ preserves $\leq$, $\neq$, 
%the function defined by
%$(x,y) \mapsto f(y,x,x)$ behaves a $\mi$,
%, $(x,y) \mapsto f(x,y,x)$, and $(x,y) \mapsto (
%and for all $x,y$ it holds that $f(y,x,x) = \alpha f(x,y,x) = \beta f(x,x,y)$. 


%Let $c_1, \dots,c_n \in \mQ$ be arbitrary. 
%Let $\mQ = Q_1 \uplus Q_1$ be a partition
%of the rational numbers into two dense subsets, and define
%$$
%g(x,y) := \left\{\begin{array}{l l l}
%a_1(x) & \text{if } x=y \in Q_1 \\
%a_2(x) & \text{if } x<y \text{ and } x \in Q_1 \\
%a_3(y) & \text{if } x>y \text{ and } y \in Q_1 \\
%a_4(y) & \text{if } x=y \in Q_2 \\
%a_5(y) & \text{if } x>y \text{ and } y \in Q_2 \\
%a_6(y) & \text{if } x<y \text{ and } x \in Q_2 
%\end{array} \right.
%$$
%where $a_1,\dots,a_6$ are unary operations that preserve $<$ 
%such that 
%\begin{itemize}
%\item $a_1(x) = x$ for all $x \in Q_1 \cap \{c_1,\dots,c_n\}$,
%\item $a_4(x) = x$ for all $x \in Q_2 \cap \{c_1,\dots,c_n\}$, and
%\item for all $x\in\mathbb{Q}$ and all
%$0<\varepsilon\in\mathbb{Q}$ 
%$$a_1(x) < \cdots < a_6(x) < a_1(x+\varepsilon) \; .$$ 
%\end{itemize}
%Operations $a_1,\dots,a_6$ with these properties can be constructed similarly as demonstrated for $\mi$ in Section~\ref{ssect:mi}. The image of 
%$g$ induces in $(\mQ;<)$ a dense linear order without 
%endpoints, and is therefore isomorphic to $(\mQ;<)$.
%When $\alpha$ is such an isomorphism, then 
%$\alpha g$ is surjective. Replacing $g$ by $\alpha g$,
%we therefore assume in the following that $g$ is surjective. 
%For an illustration of $g$, see Figure~\ref{fig:good-mi}.
%Red vertices are from $\{(x,x) \; | \; x\in Q_1\}$, 
%blue vertices from $\{(x,x) \; | \; x\in Q_2\}$.


%\begin{figure}
%\begin{center}
%\includegraphics[scale=.6]{tcsp/good-mi.pdf}
%\caption{Illustration of the operation $g$.}
%\label{fig:good-mi}
%\end{center}
%\end{figure}

%\begin{proposition}\label{prop:good-mi}
%There are $\alpha,\beta \in \Aut((\mQ;<,c_1,\dots,c_n))$
such that $g(x,y) = \alpha g(\beta y, \beta x)$ holds 
for all $x,y \in \mQ$.
\end{proposition}
\begin{proof}
Analogous to the proof of Proposition~\ref{prop:good-ll}.
\ignore{
We first show that for all finite subsets $S$ of $\mQ$
there exist automorphisms $\alpha,\beta$ of $(\mQ;<)$
such that $g(x,y) = \alpha g(\beta y, \beta x)$ for all $x,y \in S$.
Let $\{s_1,\dots,s_n\} = S$ with $s_1 < \cdots < s_n$.
By adding extra elements to $S$ we can assume without loss of
generality that $n$ is even, $s_{2i-1} \in Q_1$, and $s_{2i} \in Q_2$ for $1 \leq i \leq n/2$.
Then choose $\beta$ to be an automorphism of $(\mQ;<)$
that sends $s_i$ to $s_{i+1}$, for all $i < n$. The weak linear order induced 
by $g(\beta y, \beta x)$ on $S^2$ is the same
as the weak linear order induced by $g(x,y)$, and hence
there exists an automorphism $\alpha$
that maps $g(\beta y, \beta x)$ to $g(x,y)$ for all $x,y \in S$.

The existence of $a,b \in \End((\mQ;<))$
and $f \in \langle g \rangle$ 
such that $\forall x,y. \; f(x,y) = a(f(b(y), b(x)))$
can now be shown similarly as in the proof of Lemma~\ref{lem:lift}. 
}
\end{proof}



%Let $r_1,r_2,\dots$ be an enumeration of $\mathbb Q$. 
%Inductively assume that 
%we have already defined $a_1,\dots,a_6$ on $\{r_1,\dots, r_n\}$ such that 
%$a_1(r_i) < \cdots < a_r(r_i) < a_1(r_j)$
%whenever $r_i < r_j$, for $i,j \in [n]$.
%Clearly, this is possible for $n=1$. 
% ETC did not finish
%If $a_{n+1} > a_i$ for all $i \in [n]$, let $a_j$ be the maximum
%of $\{a_1,\dots,a_n\}$,  and define $\alpha(a_j) < \beta(a_{n+1}) < \gamma(a_{n+1}) < \alpha(a_{n+1})$.
%In the case that $a_{n+1} < a_i$ for all $i \in [n]$ we proceed analogously. Otherwise, let $i,j \in [n]$ such that
%$a_i$ is the largest possible and $a_j$ is smallest possible 
%such that $a_i<a_{n+1}<a_j$. In this case, define $\alpha(a_i) < \beta(a_{n+1}) < \gamma(a_{n+1}) < \alpha(a_{n+1}) < \beta(a_j)$.
%In this way we define unary operations
%$\alpha, \beta, \gamma$ on all of $\mathbb Q$ with the desired properties.


%So this already gives us unary operations $a,b$ and a binary
%operation $g$ such that $

%To formally describe our algorithm we need the following definitions.  Let
%$\phi=R(x_1,\dots,x_k)$ be an atomic formula where $R$ is a temporal relation
%that is preserved by an operation $f$.  Clearly, for all $x_i$ from
%$x_1,\dots,x_k$ the temporal relation defined by $\exists x_i. \phi$ is
%preserved by $f$ as well.  Therefore, if $\phi_1 \wedge \dots \wedge \phi_m$ is an instance of the CSP with
%constraints that are preserved by $f$, and $y$ is a variable from $\bar x$, 
%then $\psi := \exists y. \phi_1 \wedge \cdots \wedge \exists y. \phi_m$ can also be viewed as an instance of the CSP with constraints
%preserved by $f$.  We call $\psi$ the \emph{projection} of $\Phi$ to $X
%\setminus \bar y$. 
%Note that $\psi$ is in general not equivalent to $\exists y (\psi_1 \wedge \dots \wedge \phi_m)$. But if $\psi$ is unsatisfiable, then $\phi$ is
%unsatisfiable as well.

\ignore{ % this should be clear by now!
\begin{lemma}\label{lem:generation-relationally}
An operation $f$ generates $g$ 
if and only if every temporal relation that is preserved by $f$ is also preserved by $g$. 
\end{lemma}
\begin{proof}
By definition, $f$ generates $g$ if and only if $F = \{f\} \cup \Aut$ locally
generates $g$. Proposition~\ref{prop:locclos} shows that
this is the case if and only if $g$ preserves all relations in $\inv(F)$.
Since a relation is preserved by $\Aut$ if and only if it
is a temporal relation, we find that $g$ preserves all relations in $\inv(F)$
if and only if $g$ preserves all temporal relations preserved by $f$,
which is what we had to show.
\end{proof}}
%We now present an equivalent description of the polymorphism clone
%of a temporal constraint language that is generated by
%a single operation.
%
\ignore{First, we show that $=_I$ defines the kernel of $h$, that is,
for all $(a_1,a_2), (b_1,b_2) \in \delta(\bB^2)$ we have that 
$h(a_1,a_2) = h(b_1,b_2)$ if and only if $\bB \models =_I(a_1,a_2,b_1,b_2)$.
Suppose that $\bB \models \phi_=(a_1,a_2,b_1,b_2)$. Then either $a_1=0$ or $b_2=0$.
If $a_1=0$, then $a_2 \neq 0$, and hence $h(a_1,a_2)=h(b_1,b_2)=0$.
Similarly, if $b_2=0$, then $b_1 \neq 1$, and hence $h(a_1,a_2)=h(b_1,b_2)=1$.
Conversely, suppose that $h(a_1,a_2) = h(b_1,b_2)$. 
If $h(a_1,a_2) = h(b_1,b_2)=0$, then $a_1=b_1=0$, and $b_2 \neq 0$, 
and hence $\bB \models T_3(0,a_1,b_2)$.
If $h(a_1,a_2) = h(b_1,b_2)=1$, then $a_2=b_2=0$, and $a_1 \neq 0$, 
and hence $\bB \models T_3(0,a_1,b_2)$.
Finally, we have to show that 
%for all elements $a_1,a_2,b_1,b_2,c_1,c_2$
%of $\bB$ such that $(a_1,a_2), (b_1,b_2), (c_1,c_2)$ satisfy $\delta$ in $\bB$,
for all $(a_1,a_2), (b_1,b_2), (c_1,c_2) \in \delta(\bB^2)$ 
we have that 
$$\bB \models \phi_{\text{1IN3}}(a_1,a_2,b_1,b_2,c_1,c_2) \; 
\Leftrightarrow \; (h(a_1,a_2),h(b_1,b_2),h(c_1,c_2)) \in \text{1IN3} \; .$$
Suppose first that $\bB \models \phi_{\text{1IN3}}(a_1,a_2,b_1,b_2,c_1,c_2)$.
Let $d$ be a value for $u$ that shows that
$\bB \models \exists u. T_3(u,a_1,b_1) \wedge T_3(0,u,c_1)$; then either
$u$ or $c_1$ must be equal to $0$; if $u=0$, then either $a_1=0$ or $b_1=0$.
Hence, exactly one out of $a_1,b_1$, and $c_1$ equals $0$,
and exactly one out of $h(a_1,a_2),h(b_1,b_2),h(c_1,c_2)$ equals $0$.
%
Conversely, suppose that exactly one out of $h(a_1,a_2),h(b_1,b_2),h(c_1,c_2)$ equals $0$.
Then exactly one out of $a_1,b_1,c_1$ equals $0$, and we can set $u$ to the minimum
of $b_1$ and $c_1$ to satisfy $T_3(u,a_1,b_1) \wedge T_3(0,u,c_1)$ in $\bB$.}
%

==> tcsp/prelims.tex <==
% NOT USED ANY MORE, ALREADY INCLUDED SOMEWHERE ELSE
%\section{Preliminaries}
%\input{mt.tex} check whether everything appears in the new text
\subsection{Cameron's theorem}
\label{ssect:aut}
In this subsection we recall the classical result of Cameron~\cite{Cameron5} that describes temporal constraint languages
up to first-order interdefinability.
For $x_1,\ldots,x_n\in \mathbb{Q}$ write $\overrightarrow{x_1\ldots x_n}$ when $x_1<\ldots<x_n$. 
%Then we define a ternary relation $\Betw$ on $\mathbb{Q}$ by $\Betw:=\{(x,y,z)\in \mathbb{Q}^{3}\;|\; \overrightarrow{xyz}\vee \overrightarrow{zyx}\}$. Define another ternary relation $\Cycl$ by $\Cycl:=\{(x,y,z) \in\mathbb{Q}^{3}\;|\; \overrightarrow{xyz}\vee \overrightarrow{yzx}\vee \overrightarrow{zxy}\}$. Finally, define a $4$-ary relation $\sep$ by $\sep:=\{(x,y,z,w)\in \mathbb{Q}^{4}\;|\; \overrightarrow{xyzw}\vee \overrightarrow{wzyx}\}$.

\begin{theorem}[Relational version of Camerons theorem; see e.g.~\cite{JunkerZiegler}]\label{thm:order-reducts}
Let $\bA$ be a temporal constraint language.
Then $\bA$ is first-order interdefinable with exactly 
one out of the following five homogeneous structures.
\begin{itemize}
\item The dense linear order $(\mathbb{Q};<)$ itself,
\item The structure $(\mathbb{Q}; \btw)$, where \btw\ is the ternary relation \\
$\{(x,y,z) \in {\mathbb Q}^3 \; | \; \overrightarrow{xyz} \, \vee \,
\overrightarrow{zyx} \}$
\item The structure $(\mathbb{Q}; \Cycl)$, where \Cycl\ is the ternary
  relation \\ 
  $\{(x,y,z) \; | \; \overrightarrow{xyz} \vee \overrightarrow{yzx} \vee \overrightarrow{zxy}\}$,
\item The structure $(\mathbb{Q}; \sep)$, where \sep\ is the 4-ary relation \\
 $\{(x_1,y_1,x_2,y_2) \; | \;
  \overrightarrow{x_1x_2y_1y_2} \vee \overrightarrow{x_1y_2y_1x_2} \vee
  \overrightarrow{y_1x_2x_1y_2} \vee \overrightarrow{y_1y_2x_1x_2} \vee \overrightarrow{x_2x_1y_2y_1}
  \vee
  \overrightarrow{x_2y_1y_2x_1} \vee \overrightarrow{y_2x_1x_2y_1} \vee \overrightarrow{y_2y_1x_2x_1}\}$,
\item The structure $(\mathbb{Q};=)$.
\end{itemize}
\end{theorem}
The relation \sep\ is the so-called \emph{separation relation};
note that $\sep(x_1,y_1,x_2,y_2)$ holds for elements $x_1,y_1,x_2,y_2 \in \mathbb Q$ iff all four points $x_1,y_1,x_2,y_2$ are distinct
and the smallest interval over $\mathbb Q$ 
containing $x_1,y_1$ properly overlaps with the smallest interval containing $x_2,y_2$
(where properly overlaps means that the two intervals have a non-empty intersection, but one interval does not contain the other).

Temporal constraint languages naturally arise in the theory of infinite permutation groups,
because these structures are precisely the structures 
with a largest possible degree of symmetry on its subsets,
which is formalized with the following definition.
A subset of $D$ is called a \emph{$k$-subset} if it has cardinality $k$;
the \emph{orbit of a $k$-set} $S$ is the set
$\{ \alpha(S) \; | \; \alpha \in \text{Aut}(\bA)\}$ where $\alpha(S)$
is the image of the set $S$ under $\alpha$.

\begin{definition}
A structure $\bA$ is called \emph{highly set-transitive} if for all
$k \geq 1$ the structure $\bA$ has precisely one orbit of $k$-sets.
\end{definition}

The next theorem was also shown by Cameron~\cite{Cameron5}, and was his original motivation for the investigation of structures with a first-order definition in $(\mathbb Q; <)$. It will not be used 
in the results we present; however, we would like to state
it here because it provides a fundamentally different characterization
of the class of temporal constraint languages.

\begin{theorem}\label{thm:set-trans}
A relational structure $\bA$ is highly set-transitive if and only if it is a temporal constraint language.
\end{theorem}

